Security Threats and Cellular Network Procedures for Unmanned Aircraft Systems

This paper discusses cellular network security for unmanned aircraft systems (UASs) and provides insights into the ongoing Third Generation Partnership Project (3GPP) standardization efforts with respect to authentication and authorization, location information privacy, and command and control signaling. We introduce the 3GPP reference architecture for network connected UAS and the new network functions as part of the 5G core network, discuss introduce the three security contexts, potential threats, and the 3GPP procedures. The paper identifies research opportunities for UAS communications security and recommends critical security features and processes to be considered for standardization.

==> include/otherUAVservices.tex <==
%TC:ignore
\begin{table*}[ht]
\centering
\caption{KPIs for UAV-assisted wireless services according to 3GPP TS 22.125, V17.1.0.}%~\cite{UAS_5G}.}

{\begin{tabular}{|p{2.7cm}|p{2.38cm}|p{1.25cm}|p{1.5cm}|p{1.4cm}|p{1.3cm}|p{1.8cm}|p{2.4cm}|}
\hline
\centering
\textbf{Service} & \textbf{Uplink \newline Data rate} & \textbf{Uplink Latency} &\textbf{Downlink Data Rate} & \textbf{Downlink Latency} & \textbf{Height} &  \textbf{Service Area} &  \textbf{%\textcolor{blue}{
Use Case}%}
\\ \hline
\vspace{-0.05 in}
8K video live broadcast &
\vspace{-0.05 in}
100 Mbps
&
\vspace{-0.05 in}
200 ms
&
\vspace{-0.05 in}
600 Kbps
&
\vspace{-0.05 in}
20 ms
&
\vspace{-0.05 in}
$<$ \text{100 m}
&
\vspace{-0.05 in}
Urban, scenic area
&
\vspace{-0.05 in}
%\textcolor{blue}{
Healthcare, virtual reality%}
\\ \hline
\vspace{-0.05 in}
{4*4K AI surveillance} &
\vspace{-0.05 in}
120 Mbps
&
\vspace{-0.05 in}
20 ms
&
\vspace{-0.05 in}
50 Mbps
&
\vspace{-0.05 in}
20 ms
&
\vspace{-0.05 in}
$<$ \text{200 m}
&
\vspace{-0.05 in}
Urban, rural area
&
\vspace{-0.05 in}
%\textcolor{blue}{
Face and object recognition, environment awareness, autonomous driving%}
\\ \hline
\vspace{-0.05 in}
{Remote UAV controller through HD video} &
\vspace{-0.05 in}
$\geq$ \text{25 Mbps}
&
\vspace{-0.05 in}
100 ms
&
\vspace{-0.05 in}
300 Kbps
&
\vspace{-0.05 in}
20 ms
&
\vspace{-0.05 in}
$<$ \text{300 m}
&
\vspace{-0.05 in}
Urban, rural area
&
\vspace{-0.05 in}
%\textcolor{blue}{
Non-LoS bidirectional UAV control%} 
\\ \hline
\vspace{-0.05 in}
{Real-Time Video} &
\vspace{-0.05 in}
0.06 Mbps 
&
\vspace{-0.05 in}
100 ms
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
Urban, rural, countryside
&
\vspace{-0.05 in}
Entertainment %Enhancing user engagement and
with multiple  \newline camera views%}
\\ \hline
\vspace{-0.05 in}
{Video streaming} &
\vspace{-0.05 in}
4 Mbps$\to$  \text{720p} \newline
9 Mbps$\to$ \text{1080p}
&
\vspace{-0.05 in}
100 ms
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
Urban, rural, countryside
&
\vspace{-0.05 in}
%\textcolor{blue}{
Public safety, emergency surveillance,  law  enforcement%}
\\ \hline
\vspace{-0.05 in}
{Periodic still photos} &
\vspace{-0.05 in}
1 Mbps
&
\vspace{-0.05 in}
1 s
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
$<$ \text{120 m}
&
\vspace{-0.05 in}
Urban, rural, countryside
&
\vspace{-0.05 in}
%\textcolor{blue}{
Exploration, inspections, search \& rescue%}
\\ \hline
\end{tabular}%
}
\label{tab:KPI1}
\end{table*}
%TC:endignore
